Search for Charm-quark Production via Dimuons in Neutrino Telescopes

Dimuon events induced by charm-quark productions from neutrino deep inelastic scattering (DIS) processes have been studied in traditional DIS experiments for decades. The recent progress in neutrino telescopes makes it possible to search such dimuon events at energies far beyond laboratory scale. In this paper, we construct a simulation framework to calculate yields and distributions of dimuon signals in an IceCube-like km3 scale neutrino telescope. Due to experimental limitation in the resolution of double-track lateral distance, only dimuon produced outside the detector volume are considered. Detailed information about simulation results for ten years exposure is demonstrated. Both an earlier work [1] and our work study a similar situation, we therefore use that paper as a baseline to conduct comparisons. We then estimate the impacts of different calculation methods of muon energy losses, and find that, the average energy loss formula used in that work results in more events by contrast with Monte Carlo simulation. Finally, we study the experimental potential of dimuon searches under the hypothesis of single-muon background-only. Our results based on a simplified double-track reconstruction indicate a moderate sensitivity especially with the ORCA configuration. Further developments on both the reconstruction algorithm and possible detector designs are thus required, and are under investigation.

==> header.tex <==
\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx,tabularx}
\usepackage{color}
\usepackage{multirow}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{slashed}
\usepackage[normalem]{ulem}
\usepackage{scalerel}
\usepackage{diagbox}

\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

\newcommand{\be}{\begin{equation} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\def\figureautorefname~#1\null{Fig.\,#1\null}
\def\tableautorefname~#1\null{Tab.\,#1\null}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\def\equationautorefname~#1\null{Eq.\,(#1)\null}

% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}
\newcommand{\br}{\mathrm{BR}}

% Units
\newcommand{\ev}{\text{eV}}
\newcommand{\kev}{\text{keV}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}

\newcommand{\ab}{\text{ab}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\pb}{\text{pb}}
\newcommand{\ipb}{\text{pb}^{-1}}

\newcommand{\nm}{\text{nm}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}

\newcommand{\mrad}{\text{mrad}}
\newcommand{\murad}{\mu\text{rad}}

\newcommand{\g}{\text{g}}
\newcommand{\kg}{\text{kg}}
\newcommand{\ton}{\text{t}}
\newcommand{\sr}{\text{sr}}
\newcommand{\ns}{\text{ns}}

\newcommand{\fasernu}{FASER$\nu$~}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}

%comments
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}
%\newcommand{\changed}[2]{#2}
\newcommand{\Felix}[1]{\textcolor{magenta}{[FK: #1]}}
\newcommand{\Yue}[1]{\textcolor{blue}{[YZ: #1]}}
\newcommand{\KJK}[1]{\textcolor{red}{[KK: #1]}}
\newcommand{\Douglas}[1]{\textcolor{green}{DT: #1}}

\crefname{section}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{appendix}{Appendix}{Appendices}

%Ref Style
\bibliographystyle{utphys}


